A Study on the Prevalence of Human Values in Software Engineering Publications, 2015-2018

Failure to account for human values in software (e.g., equality and fairness) can result in user dissatisfaction and negative socio-economic impact. Engineering these values in software, however, requires technical and methodological support throughout the development life cycle. This paper investigates to what extent software engineering (SE) research has considered human values. We investigate the prevalence of human values in recent (2015 - 2018) publications at some of the top-tier SE conferences and journals. We classify SE publications, based on their relevance to different values, against a widely used value structure adopted from social sciences. Our results show that: (a) only a small proportion of the publications directly consider values, classified as relevant publications; (b) for the majority of the values, very few or no relevant publications were found; and (c) the prevalence of the relevant publications was higher in SE conferences compared to SE journals. This paper shares these and other insights that motivate research on human values in software engineering.

==> Table_ValueCat_withExamples.tex <==
\caption{Value categories with a classified abstract example}
\label{tab:valuecategories_Examples}
\centering
\begin{tabular}{|l|p{13cm}|}
\hline
\textbf{Value Category} & \textbf{Example abstract and value - if available} \\ \hline
Self-direction & \arif{Paper Id 174;179;1156} \\ \hline
Stimulation & \arif{Not found} \\ \hline
Hedonism & \arif{Not found} \\ \hline
Achievement & \arif{Paper Id 30,986} \\ \hline
Power & \arif{Paper Id 442} \\ \hline
Security & \arif{Paper Id 6; 35; 37; 295; 296; 299; 301; 302; 309; 560; 593; 704; 848; 849; 985; 1014; 1120; 1123; 1132; 1134; 1136} \\ \hline
Conformity  & \arif{Paper Id 32;157;436;441} \\ \hline
Tradition & \arif{Not Found} \\ \hline
Benevolence  & \arif{Paper Id 303;421;431;872} \\ \hline
Universalism  & Paper Id 8: \textit{... The battery power limitation of mobile devices has push developers and researchers to search for methods to improve the energy efficiency of mobile apps. We propose a multiobjective refactoring approach to automatically improve the architecture of mobile apps, while controlling for energy efficiency...} (value - protecting environment) \\ \hline
Holistic View & \arif{Paper Id 316;440;559;580;698} \\ \hline
\end{tabular}

==> Table_kappa.tex <==
\caption{The inter-rater agreement (Kappa) and its interpretation~\cite{landis1977measurement} at different classification levels.}
\label{tab:KappaValue}
\centering
\small
\begin{tabular}{lll}
\toprule
\textbf{Agreement Level}& \textbf{Kappa Value} & \textbf{Agreement Strength} \\ \midrule
(a) Relevance & 0.92 & Almost perfect \\ \hline
(b) Value Category & 0.87 & Almost perfect \\ \hline
(c) Value & 0.79 & Substantial \\ \bottomrule 
\end{tabular}


==> application.tex <==
\section{Application of the Categorization \davoud{was decided to use classification} Scheme}
We apply the above mentioned scheme in order to answer the basic research questions mention in the Introduction. As figure \ref{fig:process} shows, the main process had 4 phases as pre-categorization, applying categorization scheme, disagreement resolution and analysis. In this section we discuss first three phases followed by the analysis in the results section.
\subsection{Pre-categorization}
\subsubsection{Pilot Study and calibration}
The pilot study was done with selected 49 papers of the ICSE 2018 conference. Three raters were assigned randomly to each abstract and the all raters worked individually. At the end of the pilot study all raters got together for a calibration meeting where we took a few decisions to move forward.

 \waqar{this again is the process rather than part of the scheme itself}Based on this scheme, first, raters were asked to read a abstract and first judge whether that publication is directly related to human values or not. If it is related, then the rater would judge value category for the paper. Further, rater would judge an individual value in that category for the paper if it is possible. If both raters of the a paper have agreed as the paper is relevant to human value, then we consider it as a relevance level agreement. Following the same rule, we define the category level agreement and the individual value level agreements.
 
 However, in the field of software engineering, we do not find any practical definitions either for the value categories or the individual values \cite{Mougouei2018}. Therefore, we recognized the chance of picking an individual value(s) for a abstract which is not necessarily align with the original Schwartz's model hierarchy. Most common example was the security-privacy pair. Raters found several papers which can be categorized under the security category and which belonged to privacy as the individual value. According to Schwartz, privacy is not belong to security category but for the self direction. Therefore, we relaxed the restrictions and allowed to pick any individual values as per raters' judgment. This resulted 33 abstract classifications which go against the original Schwartz's model. The comparison of the results are discussed in the section \ref{subsec:values-consideration}. \harsha{Arif, please check the subsection number}

\begin{enumerate}[(i)]
\item Reduce the number of raters from three to two due to the resource availability.
\item As every paper has some sort of value, strictly look at the explicit link between the research and the human values in the categorization scheme. 
\item Pay more attention to the contribution they have provided, rather looking at the high-level problem they are trying to solve. 
\item Finalized the years and venues
\item Adding a new value category as holistic view as raters found some papers which have considered values as a single unit. In such case, existing Schwartz's model do not support. Therefore we have added the 11th category.
\end{enumerate}


\begin{comment}
\subsection{Research Questions \davoud{research questions have changed; see the intro}}
For the selected sample: 

\davoud{do we really need to repeat RQs here?}
\begin{itemize}
    \item \textbf{(RQ1)} What values are commonly considered? 
    \item \textbf{(RQ2)} What values are under-represented?
    \item \textbf{(RQ3)} How are the publications supporting values distributed among top-tier SE venues? 
\end{itemize}
\end{comment}


\subsubsection{Paper Collection for Categorization}
As we mentioned, among the many conference and journals in the software engineering field, we have applied our scheme for two conference (ICSE and FSE) and two journals (TSE and TOSEM) within the expand of 4 years. Except for the main tracks, we considered two other tracks from ICSE namely, Software Engineering in Practice (SEIP) and  Software Engineering in Society (SEIS). As table \ref{papercount} shows, we ended up with 1350 total number of publications.\harsha{we have to justify this selection with a proper argument and can't we enforce the paper collection table to be here?} 


\subsection{Applying categorization process}
\label{subsec:classification-process}
\ref{subsec:classification-process}
\label{sec:result-classification-process}

In the classification process, we adapted the steps provided by Bertolino, et al. \cite{Bertolino2018} \harsha{have to double check this reference for these steps} as follows:
\waqar{Should be consistent, is this categorization process or classification - also we don't apply categorization process. The heading should either say Categorization Process or Classification process and the text following it should be consistent with the heading}
\begin{enumerate}[(i)] 
    \item We had seven raters who are experts or experienced academics \harsha{have to check this?} in the domains of software engineering and human values. All 1350 papers were allocated among them randomly in a way that each paper has two raters. Couples were mixed based on the expertise such that there is always a mix of experiences in research.
    \item All supportive information was given such as Schwartz's model image and category definitions. We used an online shared spreadsheet to do the classification. 
    \item After reading the title and the abstract of each paper, the rater needs to decide whether the paper is (a) directly relevant or not relevant to human values, and, if relevant, (b) to which value categories of human values and (c) to which specific human values. As previously mentioned the value categories and individual values are derived from \cite{Schwartz2012} as shown in Figure \ref{fig_values}. 
    \item In the classification process,for (b), the rater needs to choose one value category. As for (c), the rater has the options as not to choose any specific value or choose up to three specific value. 
    \arif{in the last step, we need to inform that the arbiter is one of the remaining author. We can change all `author` terms into `raters`}.
\end{enumerate}

\arif{Harsha: do not forget to change Specific Value to Individual Value}

\begin{comment}
When we were classifying paper, we intentionally ignored the productivity and efficiency (anyway not in the model) as almost all the paper somehow related to one or both. 

We looked at the direct implications to SE community or society in general in terms of Human values

We had two raters per paper and papers were randomly allocated.

As we had 7 raters and 14 pairs - a mix of experience on the domain

High-level overview of the method given in the figure
\end{comment}



\begin{figure}[htb]
    \centering
    \includegraphics[width=7cm]{Figures/process2.png}
    \caption{Process of classification}  \waqar{we might want to say  Initial  Classification  phase -1 instead of applying categorization scheme, then the final step should be be Final Classification}
    \label{fig:process}
\end{figure} 



% \begin{table}[htb]
% \centering
% \caption{Interrater agreement and kappa value \arif{The kappa value needs to be updated: please refers to \ref{sec:result-classification-process}}}
% \label{tab:interrater-agreement}
% \begin{tabular}{llrr}
% Overall                                       & ($\kappa=0.93$)               & \multicolumn{2}{c}{Rater1}                                        \\ \cline{3-4} 
% & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{Relevant} & \multicolumn{1}{l|}{Not Relevant} \\ \cline{2-4} 
% \multicolumn{1}{c|}{\multirow{2}{*}{Rater 2}} & \multicolumn{1}{l|}{Relevant}     & \multicolumn{1}{r|}{198}      & \multicolumn{1}{r|}{17}           \\ \cline{2-4} 
% \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{Not Relevant} & \multicolumn{1}{r|}{9}        & \multicolumn{1}{r|}{1004}         \\ \cline{2-4} 
% \end{tabular}
% \end{table}







%\begin{table}[htb]
%	\begin{tabular}{|l|l|l|}
%		\hline
%		\textbf{Level} & \textbf{Classification} & \textbf{Description}                                                                                                                                                        \\ \hline
%		1        & Relevance               & The raters classify whether a paper is directly relevant or not relevant to human values.                                                                                   \\ \hline
%		2        & Value category          & The raters classify whether a paper has relevance to specific value category. This level only applicable for paper that are classified as "Directly Relevant" on Level 1.   \\ \hline
%		3        & Individual value        & The raters classify whether a paper has relevance to specific individual value. This level only applicable for paper that are classified as "Directly Relevant" on Level 1. \\ \hline
%	\end{tabular}
%\end{table}

\subsection{Disagreement Resolution}

In case of disagreements on each classification level, both raters met and discussed the disagreements. At the end of the discussion, the rater has the freedom to stand on his/her opinion or change his/her mind.

One of the remaining author acted as an arbiter to discuss with the raters and figure out the reason of the disagreement. Some of the raters change his/her opinion after having the discussion. The result of this step becomes the result of our classification. 

 176 disagreements were discussed (in all three levels) and 145 was changed (in all three levels) \harsha{We have to explain why most of them were changed. Nature of values? Or individual experience? Or why?}


\harsha{Arif, Will have a chat and present these values in a better way}
\arif{Do we have to present the exact number of the disagreement?}





==> categorization-scheme.tex <==
\section{Methodology}
\subsection{Classification Scheme}
\label{sec:Categorization_Scheme}
In order to understand the prevalence of support for human values in software engineering publications, we have categorized 1350 research publications. In this section we introduce the classification scheme selected for this study. As we explained, human values have been studied mainly in social sciences for decades. Though there are several human values representations available, we are using Schwartz universal model of human values as our classification scheme \cite{Schwartz2012,schwartz1994there} which is the most accepted model for represent human values \cite{}. \harsha{we might need a better justification}\waqar{i have briefly justified the choice of this scheme in the threats to validity section which can be used as a base and then extended for this section  }

\begin{figure*}[!htbp]
	\centering
	\centerline{\includegraphics[scale=0.725,angle=0]{Figures/values}}
	\captionsetup{margin=0.5cm}
	\caption{Value Model Across 68 Countries Based on Schwartz~\cite{schwartz2006valeurs,schwartz2004evaluating} (Adopted from \cite{ferrario2016values,holmes2011common})\davoud{Harsha, I have only found one true source for this figure and that was the psychology-related website I shared with you last time, can you please add that website to our bibliography and update ``Adopted ... with that?''}.}
	\label{fig_values}
\end{figure*}

As Figure \ref{fig_values} depicts, Schwartz model consist of 10 main value categories and 58 individual values. As per the Schwartz model, Each of the 10 categories in Schwartz model are defined based on a set of goals and contain a set of individual values. Table \ref{valuecategories} \harsha{@Arif, We have to take this table into the results section. examples should be added to the table} We have added another value category after the calibration in pilot phase of the classification process, which will be discussed in the \ref{} section.



\begin{comment}

\begin{figure}[htb]
    \centering
    \includegraphics[width=7cm]{Figures/threelayer.png}
    \caption{Categorization Process Decision Diagram \davoud{does the sequence matter? if yes, use arrows instead of lines, if not, then the whole diagram is not required, I think the sequence is not important here => suggest removing this diagram} \davoud{values -> values} }
    \label{fig:threelayer}
\end{figure} 
\end{comment}



\begin{comment}
as we found through the pilot study that some of the papers has considered all human values as a single entity. Altogether there are 11 main human values categories in the first layer. Moreover, following the Schwartz model, we have extended the categorization scheme to the next level to identify the main individual values. 58 individual values were identified and divided among the 11 value categories. 
\end{comment}



\begin{comment}
The scheme consists of 2 layers as the Human value category and the individual human value. First layer , human value categories have 10 
It urges to have three layers for the scheme. As demonstrated in Figure \ref{fig:threelayer}, first, the raters decided the relevance of the allocated papers to human values. If it was found as directly relevant, then rater should pick one main value category. After that, if it possible to differentiate any possible individual value, raters would pick one individual value. There are important protocols that we followed in each layer, which are explained in the following.

\textit{Relevance}. This is the first layer. In here, after reading the title and the abstract of the paper, raters had to decide whether this paper is directly related to human values. Raters were instructed to look for explicit links between the contribution of the paper and human values in the Schwartz model \cite{schwartz1994there,Schwartz2012}. The decision was made after the pilot study, which is explained below, where we learned two things. (i) If we are to create implicit links, every single paper has some connection with human values even though the paper was not trying to address any human values; (ii) Some paper had a motivation or a problem which related to humans or human values yet the actual contribution is far away from operationalizing any human value. 

\textit{Main Value Category}. If it was found that the paper is directly relevant to human values, then rater should pick the main value category. These categories were adopted from the Schwartz model. After the pilot study, we decided to add one main value category as Holistic view as we found that some papers have addressed human values as a whole unit. 

\textit{Individual Value}. There are 58 individual values in the Schwartz model. If it was possible to identify an individual value that has been addressed in the paper, then that paper was categorized under that value.

\subsection{Categorization scheme constraints and rules}
-\textbf{An individual value should not necessarily follow its category} 
Why?: Some definition of terms are bit different from the SE understanding of such value
E.g. Security and Privacy - not all paper about individual privacy are related to national security 

- \textbf{Only category selection was allowed}
Why?: Some values are absent on the model
E.g. Transparency, Sustainability 

- \textbf{Some individual values were mapped to the best possible match}
Why?: though some of the values are missing, we could see a direct link to an available value. 
E.g. Some security papers attributed to national security although those papers are not directly related to national security.

- \textbf{Asked raters to pick a main category and main individual value}
Why?: Hard to map, nature of the values, linked to each other

\subsection{Categorization Scheme and Examples}
\davoud{for tables, you can use https://www.tablesgenerator.com/}
Main value categories and its individual values are presented in the following table. Moreover, it includes a part of an abstract that has been categorized under the particular individual value. These phrases show examples of how human values are presented in the abstracts of software engineering publications.

\end{comment}





\begin{comment}
\begin{table*}[!htbp]
	\setlength\arrayrulewidth{1.5pt}
\caption{\arif{What if we only give some examples (but not all) value quotes? (1) we already gave the Schwartz model; (2) A lot empty space in where we cannot find a quote related to some values}}
	\label{table}
	\centering
	\input{table}
\end{table*}
\end{comment}




==> table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\large
%\normalsize
%\rowcolors{1}{}{lightmyblue}
\resizebox {0.8\textwidth }{!}{% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{tabular}{|p{5cm}|p{4cm}|p{9cm}|}
\hline
\textbf{Main Value Categories} & \textbf{Specific Values} & \textbf{Examples from abstracts} \\ \hline
\multirow{7}{5cm}{Self-direction (independent thought and action--choosing, creating, exploring.)} & Freedom &  \\ \cline{2-3} 
 & Creativity &  \\ \cline{2-3} 
 & Independent &  \\ \cline{2-3} 
 & Privacy & Paper ID 6: "... In this paper, we propose a novel approach that automatically detects privacy leaks of user-entered data for a given Android app and determines whether such leakage may violate the app's privacy policy claims ..." \\ \cline{2-3} 
 & Choosing own goals &  \\ \cline{2-3} 
 & curious &  \\ \cline{2-3} 
 & Self-respect &  \\ \hline
\multirow{3}{5cm}{Stimulation (excitement, novelty, and challenge in life.)} & An exciting life &  \\ \cline{2-3} 
 & A varied life &  \\ \cline{2-3} 
 & Daring &  \\ \hline
\multirow{3}{5cm}{Hedonism (pleasure or sensuous gratification for oneself.)} & Pleasure &  \\ \cline{2-3} 
 & Self Indulgent &  \\ \cline{2-3} 
 & Enjoying life &  \\ \hline
\multirow{5}{5cm}{Achievement (personal success through demonstrating competence according to social standards.)} & Ambitious &  \\ \cline{2-3} 
 & Influential &  \\ \cline{2-3} 
 & Capable &  \\ \cline{2-3} 
 & Successful &  \\ \cline{2-3} 
 & Intelligent &  \\ \hline
\multirow{5}{5cm}{Power (social status and prestige, control or dominance over people and resources.)} & Social power &  \\ \cline{2-3} 
 & Wealth &  \\ \cline{2-3} 
 & Authority &  \\ \cline{2-3} 
 & Preserving my public image &  \\ \cline{2-3} 
 & Social recognition &  \\ \hline
\multirow{7}{5cm}{Security (safety, harmony, and stability of society, of relationships, and of self.)} & National security &  \\ \cline{2-3} 
 & Reciprocation of favors &  \\ \cline{2-3} 
 & Family security &  \\ \cline{2-3} 
 & Sense of belonging &  \\ \cline{2-3} 
 & Social order & Paper ID 32: "... The presented study is the result of the manual analysis of 1,200 discussions related to licensing bugs carried out in issue trackers and in five legal mailing lists of open source communities ..." \\ \cline{2-3} 
 & Healthy &  \\ \cline{2-3} 
 & Clean &  \\ \hline
\multirow{4}{5cm}{Conformity (restraint of actions, inclinations, and impulses likely to upset or harm others and violate social expectations or norms.)} & Obedient &  \\ \cline{2-3} 
 & Self-discipline &  \\ \cline{2-3} 
 & Politeness &  \\ \cline{2-3} 
 & Honoring of parents and elders &  \\ \hline
\multirow{6}{5cm}{Tradition (respect, commitment, and acceptance of the customs and ideas that one's culture or religion provides.)} & Respect for tradition &  \\ \cline{2-3} 
 & Devout &  \\ \cline{2-3} 
 & Accepting my portion in life &  \\ \cline{2-3} 
 & Detachment &  \\ \cline{2-3} 
 & Humble &  \\ \cline{2-3} 
 & Moderate &  \\ \hline
\multirow{9}{5cm}{Benevolence (preserving and enhancing the welfare of those with whom one is in frequent personal contact (the 'in-group')} & Helpful &  \\ \cline{2-3} 
 & Responsible &  \\ \cline{2-3} 
 & Forgiving &  \\ \cline{2-3} 
 & Honest &  \\ \cline{2-3} 
 & Loyal &  \\ \cline{2-3} 
 & Mature love &  \\ \cline{2-3} 
 & a Spiritual Life &  \\ \cline{2-3} 
 & Meaning in Life &  \\ \cline{2-3} 
 & True friendship &  \\ \hline
\multirow{9}{5cm}{Universalism (understanding, appreciation, tolerance, and protection for the welfare of all people and for nature.)} & Equality &  \\ \cline{2-3} 
 & Unity with nature &  \\ \cline{2-3} 
 & Wisdom &  \\ \cline{2-3} 
 & Inner Harmony &  \\ \cline{2-3} 
 & A world of beauty &  \\ \cline{2-3} 
 & Social justice &  \\ \cline{2-3} 
 & Broad-minded &  \\ \cline{2-3} 
 & Protecting the environment &  \\ \cline{2-3} 
 & A world at peace &  \\ \hline
Holistic View (Consider human values as a complete model without focusing on predetermined values) &  &  \\ \hline
\end{tabular}
}


==> temp.tex <==
\section{Methodology}
\label{sec:methodology}
%================== 
%========Starting Para

%We considered the relevance of SE publications to human values 
    To investigate the prevalence of human values in SE research, we manually classified publications from top-tier SE conferences and journals based on their relevance to different values. We followed a methodology similar to that of prior classification work in SE \cite{shaw2003writing,systa2012inbreeding,montesi2008software}, which mapped trends of SE research over time in terms of topic and type of study. As with prior studies, ours was based on manual classification of paper abstracts by multiple raters. Classification based on abstracts, rather than reading the full paper, is sub-optimal but strikes a balance between accuracy and time needed for the study. All papers had multiple raters and inter-rater agreement was measured using Fleiss' Kappa \cite{landis1977measurement}. We chose to classify papers from the last four years of conferences and journals generally considered to be the top SE venues, namely, the International Conference on Software Engineering (ICSE), the ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering (ESEC/FSE), the IEEE Transactions on Software Engineering (TSE), and the ACM Transactions on Software Engineering and Methodology (TOSEM). 
    
    When conducting such a study, there are a number of key experimental design decisions that need to be taken, including: (i) how to define relevance to human values, given the imperfect and high-level nature of values definitions in the literature; (ii) how many raters to assign to each paper, and (iii) how to resolve disagreements between raters. To make choices about these design decisions, we first carried out a pilot study before carrying out the main study. Both the pilot and main study assumed SVS as the classification scheme. In total, we employed seven raters (5M,2F) with varying levels of seniority and experience in SE research, ranging from PhD students to senior Professors, and including one rater from outside the software engineering field. Note that this is a  relatively high number of raters compared to similar studies \cite{Bertolino2018, vessey2002research}.
    
    
    
%========Selected Venues and papers
%\textit{Paper Selection}. 
%Nevertheless, to avoid any misinterpretations,  whenever drawing conclusions across different venues, we have presented these tracks separately rather showing it as the accumulated results of ICSE. 
%As for the number of papers selected, we classified reasonably a higher number of papers compared to similar classification studies \cite{Bertolino2018, shaw2003writing} even though papers were selected from only four editions due to the limited resources.

%======Raters and rating process

% Seven raters were involved to manually classify the selected papers. These raters are coming from a SE background and currently working in the area of human values in SE. 

%Senior members of the raters had more than five years \harsha{not sure} of experience in domains.
% The image of SVS (figure \ref{fig:values}) and value category description (table \ref{tab:valuecategories_defOnly}) were available as supporting information for raters all the time.


%================Pilot phase
\subsection{Pilot Phase}
\label{subsec:Pilot-Phase}
The pilot phase had three steps: (i) Paper selection and allocation of papers to raters, (ii) Paper classification, and (iii) Calibration of classification decisions made by different raters. 
%\begin{comment}
The aim of the pilot phase was not to measure relevance of papers to values; rather, we had the following objectives:
\begin{itemize}
  \item To test the appropriateness of SVS as the classification scheme for SE publications
  \item To develop a common understanding regarding the meaning of human values in SE contexts
   \item To collect insights from raters to feed into the experimental design of the main study
\end{itemize}
%\end{comment}

%As shown in the figure \ref{fig:methodologysteps}, 
\textit{(i) Paper selection and allocation of papers to raters.} We randomly selected 49 papers from ICSE 2018 as our pilot phase dataset. These were equally allocated among the seven raters, with three raters per paper. Common practice is to assign two raters per paper \cite{Bertolino2018, vessey2002research}; three were assigned in the pilot to get a better understanding of how to map papers to values. ICSE was chosen as it has the broadest coverage of SE research \cite{Bertolino2018}. We chose the most recent ICSE proceedings -- 2018 at time of writing. 
%The sample was around 10\% of the number of selected publications from ICSE-main track for this study. 


\textit{(ii) Paper classification.} Raters classified papers based on their title, abstract and keywords which is an approach used in similar classification studies in SE \cite{shaw2003writing, glass2002research, Bertolino2018}. Raters were instructed to decide if a paper was ``relevant'' or ``not relevant'' to human values: relevance was deliberately left ill-defined as one of the objectives of the pilot was to influence the definition of this term in the main study. For relevant papers, raters were asked to classify the papers into one value category, and then into one value within the category. Raters were not mandated to follow the hierarchical structure of SVS: that is, they could classify a paper into value X and value category Y even if X did not belong to category Y. This was to give us a way to assess the appropriateness of the hierarchy in SVS. 
Raters carried out their classification independently. 



\textit{(iii) Calibration.} After classification, all seven raters met to discuss the classification decisions. The main objective was to calibrate decisions and use this to refine the definition of values relevance. The intention was \textit{not} to decide which rater picked the correct classification.

Following the pilot phase, we made a number of observations which were fed into experimental design of the main study.



\begin{enumerate}
\setlength{\itemsep}{0pt}
\item \textit{Observation 1:} Raters found that almost every paper could be classified into a small number of values such as \textit{helpfulness}, \textit{wisdom} or \textit{influence} because, in general, every piece of research tries to advance knowledge. Thus, an indirect argument could almost always be made why a paper is relevant to helpfulness (e.g., a paper on testing is helpful to testers), wisdom (any paper advances knowledge, thus leading to greater wisdom), or influence (e.g., a paper on an improved software process influences how software is developed). This observation illustrated the difficulty of working with vaguely defined concepts such as values, but also the importance of a better definition of relevance.  



\textit{Decision 1:} It is beyond the scope of this paper to fully and formally define all the values; hence, it was decided in the main study to use inter-rater agreement as evidence that a value was sufficiently understood in the context of a particular paper to provide confidence in the results. The definition of relevance was, however, refined for the main study. Raters were instructed not to make indirect arguments why a paper might be relevant to a value. Instead, in the main study, classification was based on ``direct relevance'' -- a paper is defined as directly relevant to a value if its main research contribution is to define, refine, measure or validate a particular value in software development. All other papers are classified as not relevant. Thus, a paper should only be classified as directly relevant to helpfulness if the research provides software tools or techniques to encourage people to be helpful towards each other. 

\item \textit{Observation 2:} Raters observed that some papers addressed values as a general concept rather than considering any specific value. An example would be a paper that presents a methodology for refining values into a software architecture. These papers should not be classified into any particular value category or value.


%\arif{Can be linked with \cite{stol2015holistic}}
\textit{Decision 2:} To facilitate classification of such papers, we introduced a new value category in the main study, which we call \textit{Holistic view}. A paper classified under Holistic View relates to values generally without focusing on any specific value (see Table \ref{tab:example}).

\item \textit{Observation 3:} Raters found that some papers should be classified under more than one value. 
\textit{Decision 3:} To accommodate such papers in the main study, raters were allowed to select up to three values.\jon{why 3} This decision is different from similar  studies in SE where raters were obliged to pick just one category \cite{bertolino2018categorization}. 

\item \textit{Observation 4:} Not surprisingly, as SVS was not developed specifically for SE, there were cases where the SVS model was not a perfect fit. We will return to this point in Section \ref{sec:conclusion} but a key point for the main study is that some raters chose a value X and value category Y even if X does not belong to Y according to SVS. A common example was the value \textit{Privacy}, which from a SE perspective is clearly aligned with the category \textit{Security}, and yet appears in \textit{Self-direction} according to SVS (see Figure \ref{fig:values}).

\textit{Decision 4:} The main study maintained the decision to allow selection of values and value categories independent of the Schwartz hierarchical structure. In Section \ref{sec:result}, we present data to show the effect this had on the results. 


%\item \textit{Observation 5:} In some cases, even though a paper can be classify into a value category, can not match with a particular value. For example, papers discuss about \textit{sustainability} can be easily classified under \textit{Universalism} value category based on the motivational goal but in SVS we can not find sustainability as a value.
%\textit{Decision:} Therefore, raters were allowed to classify only the value category where necessary.

\item \textit{Observation 5:} The pilot phase gave us an opportunity to measure how long it took raters to rate papers. We found that, on average, each rater spent four minutes per abstract. Given the number of papers in the main study (1350 -- see Table \ref{tab:papercount}), assigning three raters per paper would be infeasible.

%This was due to our planned number of papers for the classification phase which is significantly higher than the pilot phase.
\textit{Decision 5:} Out of necessity, we reduced the number of raters in the main study to two. This is consistent with the number of raters in similar studies \cite{Bertolino2018, vessey2002research, glass2002research}.
\end{enumerate}


%=========Classification Phase

\subsection{Main Study}
\label{subsec:classification-process}

Similar to the pilot study, the main study also had three phases: (i) Paper selection and allocation of papers to raters, (ii) Paper classification and (iii) Disagreement resolution. The final stage was different to the pilot study because rather than calibrating ratings to inform experimental design, some raters met to try to come to a consensus.

\textit{(i) Paper selection and allocation of papers to raters.} For the main study, we selected papers from ICSE, FSE, TSE and TOSEM over the last four years. These are the same venues used in similar paper classification studies \cite{Bertolino2018, glass2002research}. We selected all papers in TSE and TOSEM. For FSE, we used all papers from the main track, and for ICSE, we used all papers from the main track, from the Software Engineering in Practice (SEIP) track, and from the Software Engineering in Society (SEIS) track. The motivation for selecting tracks is to choose tracks which publish full research papers, not shorter papers. In total, there were 1350 papers published in the chosen venues over the years 2015--2018. This is a high sample size compared to similar studies (e.g., 976 in Bertolino et al. \cite{Bertolino2018} and 369 in Glass \cite{glass2002research}). Table \ref{tab:papercount} shows the distribution of selected papers by venue, track and year.
\begin{table}
\input{Table_Papercount.tex}
\end{table}
  The papers were randomly allocated among the seven raters, two raters per paper. Each rater received around 400 papers to classify.   We manually extracted  links for each of the 1350 papers from digital databases, and provided a spreadsheet with these links and values and value categories for raters to select from. 

\textit{(ii) Paper classification.} 
Similar to the pilot phase, raters were asked to classify papers on the basis of their title, abstract and keywords. However, the main study used a different definition of relevance, as suggested by the pilot study. Raters were asked to classify papers as directly relevant or not relevant, where the definition of direct relevance is as given in Section \ref{subsec:Pilot-Phase}. Papers found directly relevant to values were further classified into a category and then to a specific value(s). Throughout the process, raters complied with the decisions made during the \textit{calibration} phase in the pilot study.

\textit{(iii) Disagreement resolution.} Given the subjective nature of the classification, raters sometimes disagreed. This could arise at three levels:
(a) relevance level, where raters disagreed on whether a paper was directly relevant or not; (b) value category level, where raters disagreed on the choice of value category; and (c) value level, where raters disagreed on the choice of value.

%We further define them as follows: 
%\begin{enumerate}[(i)]
 %   \item relevance level - If both raters classified a publication as relevant(or not) to values OR raters has different o
  %  \item Value category level - If a publication agreed as relevant and, if both raters classified it into the same value category OR otherwise
   % \item Value level agreement - If a publication agreed as relevant and, if both raters classified it into the same value
%\end{enumerate}

%We found that there are 188 disagreements from above three levels which can be defined in the same way. In order to have an in-depth observation in these cases, we have decided to do a disagreement resolution.

To attempt to resolve these disagreements, raters met to discuss their views about why the paper in question was classified in a certain way.  If the raters could not come to an agreement, a third rater was introduced as an arbiter. The arbiter facilitated a second round of discussion, sharing his or her own views, to facilitate a consensus. However, if the disagreement persisted, the arbiter did not force a decision.
%The discussions helped raters came to a mutual understanding about human values definition and application in software engineering context for the majority of the values.



%However we observed that the classification phase was less challenging due to the decision taken at the pilot phase. For example, \harsha{need an example here}. However, at the end of the classification, there were 189 disagreements found at all three levels. In order to have an in-depth observation in these cases, we have decided to do a disagreement resolution.

%\harsha{following part should be taken to the results section:As per the the observation 4 in the pilot phase, raters have classified 33 papers regardless the given hierarchy of the SVS. We have captured these cases separately and compared the difference between rater-suggested classification and what if those 33 papers were categorized under SVS. Comparative results are presented in figure \ref{fig:value-categories-side} in the result section. } 



%\harsha{@Arif, Please check the number make sense with text}At the end of the classification, in a quick analysis, we found that 216 papers out of 1350 were agreed to be classified as directly relevant by both raters. Out of that 216 paper, 195 papers were classified into the same value category. Similarly, 188 papers were classified into the same value.  

%========Kappa Values 
Aligned with previous studies \cite{Bertolino2018}, we calculated inter-rater agreement using Fleiss' Kappa, once attempts at resolving disagreements had taken place. The results of the Kappa measure are interpreted according to the agreement strengths introduced by Landis and Koch \cite{landis1977measurement}. We achieved \textit{almost perfect} agreements on relevance level and category level with Kappa values equal to 0.92 and 0.87, respectively. The agreement of value level was found as \textit{substantial} with Kappa value equal to 0.79.  The results from the main study are further discussed in section \ref{sec:result}. 






\begin{comment}


 .  The results are shown in table \ref{tab:KappaValue}. 
%\harsha{should we explain why or should this addressed in the discussion section; Should we say about these values and its categorization according to landis and koch} 
We achieved \textit{'almost perfect'} agreement on \textit{relevance level} and \textit{category level} while the \textit{value level} agreement remained as \textit{'substantial'} (see Table \ref{tab:KappaValue})  \cite{landis1977measurement}. However, along with the agreement levels of classification scheme, the Kappa value decreases. One possible explanation for this would be the subjectivity of the definitions of values, especially in relation to their meanings in SE \cite{Mougouei2018}. The results from the classification phase is further discussed in section \ref{sec:result}.
\begin{table}[h]
\input{Table_kappa.tex}
\end{table}
\end{comment}

%==================END ***********************************************************************************************************************************************************************************************************************************
%========= ARCHIVED TEXT BELOW

\begin{comment}
\arif{Notes to Harsha about the results:
\begin{itemize}
    \item 1350 papers were classified
    \item 216 papers were classified as directly relevant
    \item from 216 papers: 129 individual values were found; one paper may classified to more than one values
    \item from 216 papers: 195 values category (proposed by the raters) were found
    \item from 216 papers: 188 values category (mapping from individual values to Schwartz values category) were found; one paper may classified to more than one values
\end{itemize}
}
\end{comment}
\begin{comment}


\label{sec:methodology}
Studying the prevalence of human values in SE research, 





 

%We have also considered two


%\harsha{Jon said: include this; using a subjective rating process (can cite a social science text showing validity of this method?) to assess relevance}. Similar to the study of \textit{categorization scheme for SE conference papers} by Bertolino et al. \cite{Bertolino2018} our Methodology comprises of two main phases: a pilot phase and a classification phase. As shown in Figure \ref{fig:methodologysteps}, in the pilot phase, we selected a subset from the whole set of publications and allocated among raters. At the end of the classification, raters met for a calibration where they discussed the challenges they faced. Based on these observations, we took decisions to tune up the classification process and the classification scheme. Afterwards, in the classification phase, all papers were allocated among raters and classified according to the updated classification scheme \harsha{or still SVS}. At the end of classification, raters met for a disagreement resolution where they exchanged their opinions and reclassified papers where necessary. For the disagreements remained, a third rater acted as an arbiter and proposed the final classification. Classified paper were analyzed and results are presented in section \ref{sec:result}. Following sub sections further explain the process we followed in pilot and classification phases.


%\waqar{We randomly selected 49 papers from ICSE 2018 and classified them in the pilot phase} In the pilot phase, we classified randomly selected 49 papers from ICSE 2018. The output \waqar{don't think we took the output into classification or maybe we need to clarify what we mean by output} of the pilot was taken to the classification Phase where we classified 1350 research publications. Following sections explain the process we followed.\waqar{maybe this paragraph should summarize our methodology without getting into how many papers were considered in each phase and then we can detail it out in the coming sections, where we capture how many papers were selected and what/what not was done.} 

%\waqar{so the summary of phases would included an abstract level overview of the phase perhaps something which is captured in the figures }
\begin{comment}

\subsection{Pilot Phase}
\label{subsec:Pilot-Phase}
We performed the pilot phase with the following objectives:
\begin{enumerate}[(i)]
\item clarifying ambiguities related to the definition of values due to unavailability of such definition in the SE context \cite{Mougouei2018}.
\item clarifying ambiguities related to SVS as the classification scheme.
\item given the subjective nature of human values, collect insights to improve the the classification process.
\end{enumerate}



\textit{Paper Selection and Allocation.} We randomly selected 49 papers from ICSE 2018 and allocated those papers among the seven raters in a way that each paper has three raters.\harsha{should we explain the background of raters?} All raters worked individually and independently. Raters were asked to read the title, abstract and keywords of a paper and classify it according to SVS. \harsha{need a reference to justify why just these three parts} SVS (figure \ref{fig:values}) and motivational goals of value categories (table \ref{tab:valuecategories_defOnly}) were available for raters all the time as supportive information.

\textit{Classification.} First, raters classified paper based on the relevance of a paper to human values. The question raised was \textit{' has this paper considered any human value or not?'}. If a particular paper found related to human values, then rater further classify it to values categories and values based on the SVS. Therefore, when classifying related papers, raters had 10 value categories and 58 values as options.

\textit{Calibration.} Due to the subjective nature of Human Values, as we expected, raters had faced challenges in the classification step. At a calibration meeting raters have shared their observations. After a discussion, a set of decision were taken and move forward as an input to the classification phase. Following are the 6 main observations and decisions taken at the calibration meeting.

\begin{enumerate}
\item \textit{Observation 1:} When classifying relevance to human values, every paper can be mapped to at least one value. For example, every research can somehow be viewed as \textit{helpful} considering the general role of research is to help advancing knowledge and propels the chosen field forward. If we consider such general contributions, obviously, such a classification does not serve the main purpose of this research.
\textit{Decision:} Therefore, raters agreed to avoid such general contributions from future classification and restricted themselves to classify papers if only they found a research to be \textit{directly relevant}. i.e. the intention or claimed contribution of the research focused on considering one or more human values.

\item \textit{Observation 2:} Raters found that some papers can be categorized under more than one human value thus falling under more than one value category. \arif{Can be linked with \cite{stol2015holistic}} \textit{Decision:} To facilitate classification of such papers, we have introduced a new value category called \textit{Holistic View} to the classification scheme. \harsha{should we elaborate more? what holistic view means?} 

\item \textit{Observation 3:} Raters found papers which had considered many values within the same value category. \textit{Decision:} Therefore, for the future classifications, raters were allowed to select up to maximum three individual values where necessary, but under the same value category.

\item \textit{Observation 4:} Given the SE engineering background, raters recognized that some of values should belongs to a different category compare to the SVS. One of the most common examples was the \textit{Security}-\textit{Privacy} pair. The raters found several papers which should be categorized under the security as the value category and privacy as the value. According to Schwartz, privacy does not belong to the security value category but for the the self-direction. \waqar{good, but need to be careful in explaining it, we need to do a good job at this one in particular , perhaps bring in why the raters thought privacy should be brought under security and not self-direction}
\textit{Decision:} Based on the argument, if it is necessary, raters were allowed to pick value category and value regardless the given hierarchy of SVS in future classifications. 

\item \textit{Observation 5:} In some cases, even though a paper can be classify into a value category, can not match with a particular value. For example, papers discuss about \textit{sustainability} can be easily classified under \textit{Universalism} value category based on the motivational goal but in SVS we can not find sustainability as a value.
\textit{Decision:} Therefore, raters were allowed to classify only the value category where necessary.

\item \textit{Observation 6:} Given the number of papers we had for the classification phase, we observed that allocating three raters a paper as resource intensive. \textit{Decision:} Therefore, we decided to reduce the number of raters to two in future classifications.
\end{enumerate}

\end{comment}
\end{comment}

\begin{comment}


\begin{enumerate}[(i)]
\item \textit{Observation:} When classifying relevance to human values, every paper has some sort of a connection to at least one value. For example, every paper we read, we may classify as \textit{Helpful} since every research is helpful somehow.\waqar{can somehow be viewed as helpful considering the general role of research is to help advance our  knowledge and propels the chosen field forward.}   Obviously, such a classification does not serve the main purpose of this research. \waqar{We agreed to avoid such general contribution for our future classification and restricted ourselves to classify papers if we found them to be directly relevant. i.e. the intention or claimed contribution of the research focused on delivering one or more human values} Similarly, some papers have the motivation related to human values but the solution provided is far away from operationalizing \waqar{no need to bring in operationalization here} any human value \cite{Mougouei2018} \arif{Did not found explanation about operationalizing human values in Intro and Background yet}.
\textit{Decision:} Therefore, when classifying papers, raters have agreed to have two checkpoints: (a) look for an explicit link between the main contribution of the paper to any values category or at least one value; (b) not just to look at the high-level problem that publication addresses, but has the given solution  significantly impact \arif{reviewer may asks what does it mean by significantly impact}\waqar{ditto arif} to any human value? \waqar{Raters agreed to classify a publication as directly relevant to human values }If a publication has passed both checkpoints, then it was classified as a \waqar{if it passed both checkpoints}\textit{directly relevant} publication to human values. 
\item \textit{Observation:} Some of the papers had considered a collection of human values and categories \waqar{more than one human value thus falling under more than one value category }as a single entity \arif{What does it mean by 'single entity'? Can be linked with \cite{stol2015holistic}}. \textit{Decision:} To facilitate \waqar{classification of} such papers, we have introduced a new value category called \textit{Holistic View} to the classification scheme. \waqar{can we have the heading as Observation 1 or something??}
\item \textit{Observation:} we recognized the chance of picking a value category and the value for an abstract which is not necessarily aligned with the original Schwartz's model hierarchy. One of the most common examples was the \textit{Security}-\textit{Privacy} pair. The raters found several papers which can be categorized under the security value category and which belonged to privacy as the value. According to Schwartz, privacy does not belong to the security value category but for the the self-direction.
\textit{Decision:} Therefore, if raters see it is necessary, they were allowed to pick values category and values irrespective to the given hierarchy of SVS.
\item \textit{Observation:} Some of the papers may have considered many individual values at the same time. \textit{Decision} Then, raters agreed to select up to maximum three individual values where necessary, but just one value category. \waqar{bringing the observations related to more than one value category consideration together}
\item \textit{Observation:} In some cases, even though a paper can be classify into a value category, can not match with a particular value. Some of the values such as sustainability, productivity, efficiency are not available in the SVS. \waqar{good, but need to be careful in explaining it, we need to do a good job at this one in particular , perhaps bring in why the raters thought privacy should be brought under security and not self-direction} \textit{Decision} Therefore, raters \waqar{were}allowed to classify only the value category where necessary. 
\item \textit{Observation:} Having three raters \waqar{do we need a break in the sentence here, unclear at the moment}a paper is resource consuming and hard to observe any total agreements on relevance or any other level. \textit{Decision:} Therefore, number of raters a paper would be reduced to be two. \waqar{rephrase-grammar}
\end{enumerate}


\end{comment}





%in three classification levels\waqar{3 classification levels?}. First, whether the paper is related to any human value or not? If yes, second, to which value category and finally to which value? In second and third levels, we used Schwartz universal model of human values as our classification scheme \cite{Schwartz2012, schwartz1994there}. .
%\arif{I would suggest using number: (i) whether the paper is related ..., If yes (ii) to which value category ... and (iii) to which  individual value ...}


%\waqar{Calibration?????}
%After the classification, at a calibration meeting, following decisions were taken based on the observations of the pilot study. 


%\arif{Question: should we standardize the writing of the value/category by using \textit{Value-name} and \textit{Category-name}?}

\begin{comment}


\subsection{Classification Process}
\label{subsec:classification-process}

Complying with decisions of the pilot phase, we started the classification phase. As depicts in figure \ref{fig:methodologysteps}, classification phase also had three steps.

\textit{Paper Selection and Allocation.} We have considered 1350 SE publications from four top-tier SE venues (two journals and two conferences) as our sample which were published during four years, 2015 to 2018. We have considered main tracks of ICSE and FSE as well as two additional track of ICSE (SEIS and SEIP) \harsha{Why?? We have to justify}. Paper distribution against tracks and years are shown in table \ref{tab:papercount}.


First, we have manually extracted 1350 links of research papers from databases such as ACM digital library and IEEE Xplore digital library. Then, considering research experience and domain knowledge, we have prepared 14 pairs of raters using seven raters available. Using an online worksheet, each pair was randomly allocated to papers in a way that every rater will get nearly an equal number of papers (around 400) to classify. All raters worked individually and independently.  

\textit{Paper Classification.} Similarly to the pilot phase, raters were asked to do the classification in three levels - (a) relevance, (b) values category and (c) values. Based on the decision took at pilot phase, raters were more attentive towards intention and contribution when classifying a paper as directly relevant. In the next two levels, raters still used the SVS but with the holistic view as an added value category. SVS image (figure \ref{fig:values}) and Value category description (table \ref{tab:valuecategories_defOnly}) were available as supporting information. \harsha{following part can be taken to the results section} As per the the observation 4 in the pilot phase, raters have classified 33 papers regardless the given categorization of the SVS. We have captured these cases separately and compared the difference between rater-suggested classification and what if those 33 papers were categorized under SVS. Comparative results are presented in figure \ref{fig:value-categories-side} in the result section.

If both raters agree on their opinions at any level of classification, we consider it as an agreement at that level. Consequently, there are three levels of agreements aligned with three levels of classification. At the end of the classification there were 176 disagreements found at all three levels. In order to have an in-depth observation in these cases, we have decided to do a disagreement resolution.   

\textit{Disagreement Resolution.}
In case of a disagreement at any classification level, both raters met and discussed the disagreements. At the end of the discussion, the rater had the freedom to stand on the previous opinion or change it. One of the remaining authors acted as an arbiter to discuss with the raters and figure out the reason(s) for the disagreement. Some of the raters change their opinions after having the discussion.During this discussion, the raters discussed the definitions of values in software engineering. The discussion helped raters came to a mutual understanding about human values definition in software engineering context for the majority of the values. By the end of this step, 145 disagreements were sorted out of 176. 

\harsha{@Arif, Please check the number make sense with text}At the end of the classification, in a quick analysis, we found that 216 papers out of 1350 were agreed to be classified as directly relevant by both raters. Out of that 216 paper, 195 papers were classified into the same value category. Similarly, 188 papers were classified into the same value. In order to observe the inter-rater agreement, we calculated Fleiss' Kappa on all three levels of agreement and results are shown in table \ref{tab:KappaValue}. \harsha{why this kappa value?}
\arif{Fleiss' kappa support more than two raters, while Cohen's kappa only support two raters. In reality, we have two raters, but the raters were different on each paper.}

\begin{table}[h]
\input{Table_kappa.tex}
\end{table}

\harsha{should we explain why or should this addressed in the discussion section; Should we say about these values and its categorization according to landis and koch}  


These kappa values are insightful as it leads to a broader discussion on availability of definitions for value in SE. Classify a paper on relevance has a significant level of agreement of 0.92 where it is easy to decide whether a publication has explicitly considered human values. Once we go inside the classification scheme where we find value categories and values, we can see the level of agreement goes down. This was due to the subjectivity of the definitions of the values \cite{Mougouei2018}, especially in relation to their meanings in SE. We, moreover, had to exclude 2\% of the papers (classified as undecided as in Figure \ref{fig:relevant}) from our analysis as an agreement was not reached about them, at the relevance level. Thus, subjectivity of human values has been widely recognized in social sciences~\cite{Schwartz2012} as well as in software engineering~\cite{Mougouei2018}.


%inter-rater agreement to measure the degree of agreement between the raters using Fleiss' Kappa \cite{fleiss1971measuring}.
%In step \emph{(ii)}, we achieved 0.91 Kappa value on classification (a). After step \emph{(iii)}, 

%the Kappa values are 0.92 (increase) on classification (a), 0.87 on classification (b) for the value category, and 0.75 on classification (c) for the specific value. 
%\arif{TODO: update the kappa value for Specific Value classification}
%The association of Kappa value and the strength of the agreements are defined by Landis and Koch \cite{landis1977measurement} as \emph{poor} (the Kappa value is less than 0), \emph{slight} (0 - 0.20), \emph{fair} (0.21 - 0.40), \emph{moderate} (0.41 - 0.60), \emph{substantial} (0.61 - 0.80), and \emph{almost perfect} (0.81 - 1.00).
%Thus, our classification agreements are \emph{almost perfect} for classification (a) and (b), respectively, and \emph{substantial} for classification (c). 

%Achieving a strong level of inter-rater agreements might be due to the fact that the raters, after their discussions, shared their understanding of different values in SVS.
%The discussion that the raters and the arbiter had during the classification process helped shape the definition of human values, but there are still several cases of disagreement left.
% Nevertheless, there were still cases of disagreements exists.
% the arbiter found vagueness in definitions of some human values \cite{Mougouei2018} as the primary source of disagreements among the raters.  
\end{comment}
%The final results after the disagreement resolution is considered as the final classification of 1350 papers into 11 value categories and 58 distinct values. The analysis and results of the final classification is discussed further in the section \ref{sec:result}.


%If both raters agreed upon relevance, we have considered that paper as a directly relevant paper. Within directly relevant paper we had two levels of agreements as value category level agreement and value level agreement. Analysis and the results were done and presented according to these three levels of agreements. 


%\waqar{I think this paragraph is more suited to the methodology or even discussion section rather  in the results section}. \arif{yes, I can agree with that. I put it on the Discussion section.}\waqar{reading it again in conjunction with the preceding text, it does not belong in the discussion section so lets move it somewhere in the methodology @Harsha, see where does it fit and how much of it can be used}
%During the classification process, the raters discussed the definitions of values in software engineering. The discussion helped raters came to a mutual understanding about human values definition in software engineering context for the majority of the values. This led to 87\% inter-rater agreement of paper relevance to the value categories. Also, 75\% inter-rater agreement was reached for the classification based on the specific values. Nonetheless, a full agreement was not reached neither for the value categories nor the specific values. We found subjectivity of the definitions of the values~\cite{Mougouei2018}, especially in relation to their meanings in SE, as the primary cause of such disagreements. We, moreover, had to exclude 2\% of the papers (classified as undecided as in Figure~\ref{fig:supporting-agreement}) from our analysis as an agreement was not reached about them, regarding their relevance for values. Subjectivity of human values has been widely recognized in social sciences~\cite{Schwartz2012} as well as in software engineering~\cite{Mougouei2018}. 

\begin{comment}
\begin{figure}[h]
    \centering
    \includegraphics[width=6cm]{Figures/Classificatioprocess.png}
    \caption{Classification process \davoud{low quality pic and large fonts}}
    \label{fig:Classifysteps}
\end{figure}
\end{comment}

\input{table-example}
\begin{comment}


\begin{figure}[h]
    \centering
    \hspace{0.7cm}\includegraphics[width=0.35\textwidth]{Figures/methodology.png}
    \caption{Methodology phases and steps} %\davoud{the resolutions are not great and the fonts are too big}\harsha{Shall we keep this for the moment, I am working on drawing these using a latex package; \davoud{yes you can use TikZ library}}}
    \label{fig:methodologysteps}
\end{figure} 
\end{comment}
